Hardware Functional Obfuscation With Ferroelectric Active Interconnects

Camouflaging gate techniques are typically used in hardware security to prevent reverse engineering. Layout level camouflaging by adding dummy contacts ensures some level of protection against extracting the correct netlist. Threshold voltage manipulation for multi-functional logic with identical layouts has also been introduced for functional obfuscation. All these techniques are implemented at the expense of circuit-complexity and with significant area, energy, and delay penalty. In this paper, we propose an efficient hardware encryption technique with minimal complexity and overheads based on ferroelectric field-effect transistor (FeFET) active interconnects. The active interconnect provides run-time reconfigurable inverter-buffer logic by utilizing the threshold voltage programmability of the FeFETs. Our method utilizes only two FeFETs and an inverter to realize the masking function compared to recent reconfigurable logic gate implementations using several FeFETs and complex differential logic. We fabricate the proposed circuit and demonstrate the functionality. Judicious placement of the proposed logic in the IC makes it acts as a hardware encryption key and enables encoding and decoding of the functional output without affecting the critical path timing delay. Also, we achieve comparable encryption probability with a limited number of encryption units. In addition, we show a peripheral programming scheme for reconfigurable logic by reusing the existing scan chain logic, hence obviating the need for specialized programming logic and circuitry for keybit distribution. Our analysis shows an average encryption probability of 97.43% with an increase of 2.24%/ 3.67% delay for the most critical path/ sum of 100 critical paths delay for ISCAS85 benchmarks.

==> bibtex/sections/FEFET_technology.tex <==

\section*{FeFET technology,\textcolor{blue}{repetition,move to introduction}
}\\
%\textcolor{red}{flow needs to be changes here}
%We are proposing two different approach to the problem, one is a improvement from previous work that we reduce the functionality of the circuit. 
\begin{figure}
\centering
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[scale=0.5,width=\columnwidth]{bibtex/figures/FeFET.png}
\caption{\label{Fig:FeFET}}
\end{subfigure}
\hspace{10mm}
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[scale=0.5,width=\columnwidth]{bibtex/figures/Vt.png}
\caption{\label{Fig:VT}}
\end{subfigure}
\hspace{10mm}
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[scale=0.8, width=\columnwidth]{bibtex/figures/reconf_circuit.png}
\caption{ \textcolor{blue}{first two figures are redundant,}\label{Fig:reconfig}}
\end{subfigure}
\hspace{10mm}
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[scale=0.3, width=\columnwidth]{bibtex/figures/replace_prevwork.png}
\caption{\label{Fig:Prevwork}}
\end{subfigure}

\caption{(a) Structure of FeFET (b) Reconfigurable characteristics of FeFETs by applying programming voltages \textcolor{red}{Prof Kai s comment, For the Id-Vg curve, You do not need to show both the reset and set one as they are the same.will need to double check, exactly what he meant} (c) Our proposed reconfigurable encoding circuit with FeFET-based pass transistors (d) FeFET based generic 2 input TVD camouflage circuit. This circuit can can implement NOR NAND and XOR function \cite{Mai'16}.}
\end{figure}



Ferroelectric FET (FeFET) is a MOSFET with an embedded ferroelectric layer at the MOSFET gate stack, as illustrated in Fig. \ref{fig:overview}(a),b. Ferroelectric FET exhibits many outstanding features, such as zero standby power, moderate write speed, excellent process compatibility, and scaling capability. FeFET already demonstrated promising performance in many memory-based fields \cite{Ma'16, Xueqing'18, Lai'18}, for instance, memory-centric computing and database systems. Besides, the polarization state of the ferroelectric layer can be modulated by applying different external gate voltage. Accordingly, FeFETs can achieve a tunable and stable threshold voltage V$_T$ and operation voltage adaptability. 
The key idea behind our proposed reconfigurable encoding circuit is based on voltage-dependent switching of ferroelectric polarization in the gate stack \cite{IEDM'16, IEDM'17, IEDM'181, Jerry_2018, Kai'18}. As shown in Fig. \ref{fig:overview}(c), by applying a positive programming voltage (V$_P$) greater than its coercive voltage to the gate, the polarization in ferroelectric domain would be switched and FeFET would be set to LVT state. Similarly, applying a negative erase voltage (-V$_P$) would switch the polarization toward an opposite direction and sets the transistor to HVT state. Based on the abovementioned switching principle, the feature of reconfigurability implementing many logic functionalities (e.g. AND and OR) can be achieved with a suitable choice of external gate voltages on FeFETs.



==> bibtex/sections/Fabrication_details.tex <==
\section*{Experimental Fabrication  Evaluations}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{bibtex/figures/fig11.png}
    \caption{a.Caption b.Caption c.Caption d.Caption e.Caption f.Caption g.Caption h.Caption}
    \label{fig:fig11}
\end{figure}


\begin{comment}
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.45\columnwidth}
    
    \centering
  \includegraphics[width=\columnwidth]{bibtex/figures/fig1.png}
   \caption{\label{Fig:Fabcircuit}  }
   
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\columnwidth}
    \centering
  \includegraphics[width=\columnwidth]{bibtex/figures/Fab2.png}
   \caption{\label{Fig:Fab2}}
   
    \end{subfigure}
   \begin{subfigure}[b]{0.45\columnwidth}
    \centering
  \includegraphics[width=\columnwidth]{bibtex/figures/Fab1.png}
   \caption{\label{Fig:Fab1}  }
   
   \end{subfigure}
   \hfill
   \begin{subfigure}[b]{0.45\columnwidth}
    \centering
  \includegraphics[width=\columnwidth]{bibtex/figures/Fab3.png}
   \caption{\label{Fig:Fab3}}
   \end{subfigure} 
    
    \caption{(a) Circuit Setup for experimentally evaluation. (b) Drain current in HVT mode. (c) V$_{out}$ in HVT mode. (d) V$_{out}$ in LVT mode.}
    \label{fig:my_label}
\end{figure}
\end{comment}





\begin{comment}
\begin{figure}[!ht]
  \centering
  \includegraphics[scale=0.3, width=05\columnwidth]{bibtex/figures/Fab_circuit.png}
   \caption{\label{Fig:Fabcircuit}  \textcolor{red}{Circuit setup for experimental evaluation }}
\end{figure}

Fig.~\ref{Fig:fig11} shows FeFET programmed to HVT. \textcolor{red}{
Fig.~\ref{Fig:fig11} shows XX, . Fig.~\ref{Fig:fig11} shows XX. Fig.~\ref{Fig:fig11}Shows 
XXX}


\begin{figure}
  \centering
  \includegraphics[scale=0.7, width=0.7\columnwidth]{bibtex/figures/Fab2.png}
   \caption{\label{Fig:fig11}  \textcolor{red}{ID in HVT mode }}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[scale=0.7, width=0.7\columnwidth]{bibtex/figures/Fab1.png}
   \caption{\label{Fig:fig11}  \textcolor{red}{Vout in HVT mode }}
\end{figure}

\begin{figure}[!ht]
  \centering
  \includegraphics[scale=0.7, width=0.7\columnwidth]{bibtex/figures/Fab3.png}
   \caption{\label{Fig:fig11}  \textcolor{red}{Vout in LVT mode }}
\end{figure}

\begin{figure}[!ht]
  \centering
  \includegraphics[scale=0.7, width=0.7\columnwidth]{bibtex/figures/Fab4.png}
   \caption{\label{Fig:fig11}  \textcolor{red}{ID in XX1 mode }}
\end{figure}
\end{comment}

We have done the fabrication to corroborate the proof of the proposed reconfigurable security logic concept. Fig. \ref{Fig:Fabcircuit} shows the experimental setup. Here we demonstrate the reconfigurablility through the single branch. The circuit consists of one N-Ferroelectric FET and one inverter. The voltage output of the inverter and drain current are measured. The idea is to program the FeFET to a HVT or LVT state to act as a pass transistor. In normal operation mode, the Gate voltage should be set at a suitable value which is higher than low V$_T$ and lower than high V$_T$. If the transistor is programmed to HVT, the input cannot get transferred to the drain of the transistor,which is equivalent to setting the pass transistor to a block state. If programmed to LVT, the NFEFET acts as a pass transistor in ON state, and the input gets transferred to drain terminal and the following inverter gets the output switched. We use the Programming voltage (V$_P$) - 4 V to set to high V$_T$ and + 4 V to set to Low V$_T$ with the pulsewidth of \textcolor{red}{1 us}. Note, the read phase does not require to switch the polarization and can be faster unlike the programming phase. In this experiment, in the read phase,  V$_A$ is set to 1V, V$_{CNTL}$ is set to 1 V and V$_{DD}$ is set to 1.5V.

\noindent Fig. \ref{fig:my_label}(b) shows the I$_D$ - V$_G$ characteristics of FeFET under different threshold voltage modes (LVT/HVT). And Fig. \ref{fig:my_label}(c) and Fig. \ref{fig:my_label}(d) show the values of output voltages after being programmed to HVT and LVT states under the above experiment setup. As we can see, when The FeFET is set to LVT state, then with the given control and input signals it turns to ON state and passes the value of A. Finally, the circuit outputs $\bar{A}$ through an inverter. However, if the pass transistor is set to HVT state, the given input signal is not large enough to turn it on. Thus, A cannot be passed out as shown in Fig. \ref{fig:my_label}(c).




==> bibtex/sections/circuit_analysis.tex <==


\section*{Circuit analysis}

%\subsection*{Simulation Methodology}
\subsection{Functional Verification}
%\newline
\begin{table}
\caption{ Simulation Parameters}
\begin{adjustbox}{width=0.5\columnwidth,height=0.13\textheight,center}

\centering
\begin{tabular}{|c|c|}
\hline
Technology &  45 nm  \\ %14 nm     \\
\hline
Width & 90nm   \\
\hline
Thickess of the ferroelectric & 8 nm   \\
\hline
Number of domains & 20   \\
\hline
Supply Voltage & 0.8 V  \\%0.8 V   \\
\hline
CNTL (Logic)  & 1.1 V  \\%1.1 V \\
\hline
V$_P$, pulsewidth & $\pm$ 4 V, 500 ns  \\
\hline
In & 0.8 V  \\
\hline
\end{tabular}
\label{table:parameters}
\end{adjustbox}
\end{table}

% \begin{table}
%     \centering
%     \caption{The programming strategies of peripheral circuits}
%     \begin{adjustbox}{width=0.4\columnwidth,height=0.12\textheight,center}
%     \begin{tabular}{|c|c|c|c|}
%     \hline
    
%   \multirow{2}{*}{Mode}  & \multicolumn{2}{|c|}{Programming} &  \multirow{2}{*}{Logic} \\
% \cline{2-3}
%          &  Step 1 & Step 2 & \\
%     \hline
%   L1(V$_1$)    & -4 V & +4 V & 0.8 V \\
%     \hline
%     L2 (V$_2$)    & -4 V & +4 V & 0.8 V \\ 
%     \hline
%     L3   & +4 V & GND & 1.1 V \\
%     \hline
%     L4   & GND & GND & 1.1V  \\
%     \hline
%     L5    & GND & +4  & GND  \\
%     \hline
%     \end{tabular}
%      \end{adjustbox}
%     \label{tab:peripheral_programming_strategy}
% \end{table}

  \begin{table}{\textwidth}
  \centering
   \captionof{table}{Truth table of NAND based reconfigurable logic}
   \begin{adjustbox}{width=1.1\columnwidth,height=0.12\textheight,center}
  \begin{tabular}{|c|c|c|c|c|c|}
      \hline
      INPUT1   &  INPUT2 & \begin{tabular}[c]{@{}1@{}}NAND\\(C1=BUF, C2=BUF,\\C3=BUF) \end{tabular}& \begin{tabular}[c]{@{}1@{}}AND\\ (C1=BUF, C2=BUF,\\C3=INV) \end{tabular} & \begin{tabular}[c]{@{}1@{}}OR\\ (C1=INV, C2=INV,\\C3=BUF) \end{tabular}&\begin{tabular}[c]{@{}1@{}}NOR\\ (C1=INV, C2=INV,\\C3=INV) \end{tabular}\\
    \hline
    0 & 0 & 1 & 0 & 0 & 1\\
    \hline
    0 & 1 & 1 & 0 & 1 & 0\\
    \hline
    1 & 0 & 1 & 0 & 1 & 0\\
    \hline
    1 & 1 & 0 & 1 & 1 & 0\\
    \hline
    \end{tabular}
   
    \label{tab:truth table of NAND_camouflage}
    \end{adjustbox}
  \end{table}
  
  
  
We use SPICE simulations to verify the functional correctness of the proposed reconfigurable buffer-inverter encryption block. Schematic of our proposed circuit is given in Fig.~\ref{fig:figure2_fefet}(e). We show simulations in both  buffer and inverter  mode configurations (Fig.~\ref{fig:figure2_fefet}(g),(i)).


We use spectre for our simulations. Table.~\ref{table:parameters} shows simulation parameters. We use 45nm PTM technology\cite{freepdk45} for the analysis. In the program mode, we set threshold states  of two FeFET pass transistors by applying  programming(write) voltages. In this analysis, we use a programming pulse  (V$_P$ $\pm$4 V) with a pulsewidth of 500 ns.
 In the logic mode, we assert an INPUT signal (0.8 V) at In and  control signal (CNTL1 and CNTL2) on the gate of pass transistors. We set the CNTL voltage (1.1 V)  to be higher than LVT and lower than HVT in the logic mode. 


In the inverter mode of encryption, we program  T1  to LVT by asserting $+$V$_P$ at CNTL1 and T2 to HVT by asserting $-$V$_P$ at CNTL2 terminal (Fig.~\ref{fig:overview}(h)).
  The internal polarization of both FeFETs  can be seen in the Fig.~\ref{fig:figure2_fefet}(i).
In the logic mode, we assert a read voltage (1.1 V)  at both CNTL1 and CNTL2 .  Logic input is set at 0.8 V for logic high and 0 V for logic low. The output (Out) follows a logically inverted input  (In) (Fig.~\ref{fig:figure2_fefet}(i)). 

In the buffer mode of encryption, we program  T1 to  HVT  and T2 to LVT by asserting  write voltages in  CNTL1 and CNTL2  terminals (Fig.~\ref{fig:figure2_fefet}(f)). In the logic (evaluation) mode, we assert read voltage ( 1.1 V) at both CNTLs   and output(Out) follows input (In) (Fig.~\ref{fig:figure2_fefet}(g)).  In summary, the proposed encryption circuit with same input results in two different logical outputs based on FeFETs' programmed states making it a strong candidate for reverse engineering resilient hardware (Fig.~\ref{fig:figure2_fefet}(g),(i)).
 Encryption probability and  timing beneficial placement and encryption probability is discussed in the next section. 

%Traditional  circuit encryption is to implement look-alike layout or insert dummy connection that interference with computer vision software.%Circuit camouflage integration for hardware IP protection

%\subsection*{Functional Verification}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.3\columnwidth}
%     \centering
%   \includegraphics[width=\columnwidth]{bibtex/figures/buffer_waveform.png}
%   \caption{\label{Fig:Functionalwav_1}}
%     \end{subfigure}
%   \hspace{10mm}
%   \begin{subfigure}{0.3\columnwidth}
%     \centering
%   \includegraphics[scale=0.5,width=\columnwidth]{bibtex/figures/Pr_buffer.png}
%   \caption{\label{Fig:Pr_buffer}}
%     \end{subfigure}
    
%     \begin{subfigure}{0.3\columnwidth}
%     \centering
%     \includegraphics[scale=0.5,width=\columnwidth]{bibtex/figures/inverter_waveform.png}
%     \caption{\label{Fig:Functionalwav_2} }
%     \end{subfigure}
%     \hspace{10mm}
%     \begin{subfigure}{0.3\columnwidth}
%     \centering
%   \includegraphics[scale=0.5,width=\columnwidth]{bibtex/figures/Pr_inverter.png}
%   \caption{\label{Fig:Pr_inverter}}
%     \end{subfigure}
    
%     \caption{(a) Simulated waveforms for buffer function verification (b) Simulated waveforms for programming stage of buffer function (c) Simulated waveforms for inverter function verification (d) Simulated waveforms for programming stage of inverter function, \textcolor{red}{Can you combine this to one single continuous figure in the simulation itself, also show cntl voltage} } 
% \end{figure}

 

 






\begin{comment}
\subsection{Variation Analysis}
\textcolor{red}{move to Supplementary?}

We do a variation analysis to study the delay impact on our proposed circuit.
%We utilize one 45nm nmos transistor to model and evaluate the variation study on FeFETs. 
We plot I$_{d}$-V$_{g}$ characteristics of a calibrated NMOS transistor  for the equivalent FeFET in  LVT $/$ HVT  modes in Fig.~\ref{Fig:figure3_variation_layout}(a).  We do  Monte Carlo simulations accounting for threshold voltage  gaussian variation.   Fig.~\ref{Fig:figure3_variation_layout}(b) shows the delay variation for the inverter and buffer. The probabilistic  distribution for the buffer delay and inverter delay with respect to threshold voltage variation is given in Fig.~\ref{Fig:figure3_variation_layout}(c),(d) respectively.
\end{comment}
%We observe a delay variation in the range from 16.2\% to 74.4\% for buffer and 15.3\% to 28.8\% for inverter.


%with varying its model parameters-gate oxide thickness and threshold voltage for
%The left bunch of curves are all in LVT state, which indicates they have relatively low threshold voltages. And the right bunch of curves are in HVT state and have relatively high threshold voltages. With these information, we are able to obtain an equivalent transistor with our simulated FeFET. Further, Fig.~\ref{Fig:figure3_variation_layout}b demonstrates delay of our proposed reconfigurable encoding circuit by replacing FeFETs with the equivalent transistor. We also measured the corresponding delay of the reconfigurable encoding circuit with V$_t$ following Gaussian distribution as shown in Fig.~\ref{Fig:figure3_variation_layout}c,d.




==> bibtex/sections/circuits.tex <==
\section*{Circuits\textcolor{blue}{repetition,move to introduction}}
The key operating principle for FeFET-based encryption method is based on threshold voltage switching caused by the polarization of ferroelectric layer on the gate stack. % cite for some ferroelectric paper
By applying a positive voltage or a negative voltage on the gate, the threshold voltage of the FeFET can be set to a high or low state. As shown in Fig. \ref{Fig:VT}, a positive set voltage on the gate of FeFET towards the channel and set to a LVT state. Applying a negative voltage biased the polarisation to the gate and set the transistor to HVT state. By doing this we can reconfigure the function of FeFET between a pass transistor and a circuit breaker. \par
The schematic of the FeFET based encryption circuit is shown in Fig. \ref{Fig:reconfig}. Two FeFET pass transistors are programmed into two opposite states and connected into input A and inverted input $\bar{A}$. Since the state of the pass transistors are always opposite, only one input can connect to the output hence the circuit could be reconfigured into either an inverter or a buffer. The CNTL signal is connected to the gate of two FeFETs. At setup, CNTL signal is connected to setup source, this paper uses a 4V and - 4V source to program the states of FeFETs. After the programming state, CNTL signal can either connect to VDD for part of a combination logic or connect to the clock signal to latch the input signal.



==> bibtex/sections/copy.tex <==
\section*{Background \& Motivation}


\begin{figure}
   \centering
    \includegraphics[scale=1,width=\textwidth]{bibtex/figures/figure1_overview.pdf}
     \includegraphics[width=1\textwidth]{bibtex/figures/experimental_mw.pdf}
    %\caption{Caption}
    \label{fig:overview}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{bibtex/figures/experimental_mw.pdf}
    %\caption{Caption}
    \label{fig:experimental_mw}
\end{figure}

\vspace{-3cm}

\begin{figure}

\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[scale =0.35,width=\textwidth]{bibtex/figures/our_config.png}
%\caption{default}
\label{fig:figure1.1}
\end{minipage}
%\vspace{-8cm}
\begin{minipage}[b]{0.4\linewidth}
\centering
\vspace{0.0cm}
\includegraphics[scale =1.5,width=1.5\textwidth]{bibtex/figures/ourconfig_bufinv.png}
%\caption{default}
\label{fig:figure1}
\end{minipage}

%\hspace{0.2cm}

\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{bibtex/figures/experimental_inv_buff.pdf}
   % \caption{Caption}
    \label{fig:experimental_inv_buff}
\end{figure}

\vspace{-1cm}
\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{bibtex/figures/Other_applications.pdf}
    \caption{Caption}
    \label{fig:other_applications}
\end{figure}



\begin{comment}
\begin{figure}[t]
\begin{minipage}[b]{0.2\linewidth}
\vspace{-2cm}
%\centering
\includegraphics[width=\textwidth]{bibtex/figures/ourconfig.png}
\caption{default}
\label{fig:figure1}
\end{minipage}
\hspace{0.2cm}
\begin{minipage}[b]{0.8\linewidth}
\centering
\includegraphics[width=\textwidth]{bibtex/figures/Other_applications.pdf}
\caption{default}
\label{fig:figure2}
\end{minipage}
\end{figure}


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.25\textwidth}
    \includegraphics[scale=1,width=1\textwidth]{bibtex/figures/our config.png}
    \caption{Caption}
    \label{fig:our config}
      \end{subfigure}
      
      \begin{subfigure}[b]{0.7\textwidth}
     \includegraphics[width=1\textwidth]{bibtex/figures/Other_applications.pdf}
    \caption{Caption}
    \label{fig:other_application}
    \end{subfigure}
\end{figure}
\end{comment}



% \begin{figure}[ht]
%   \centering
% %   \begin{subfigure}[b]{0.6\textwidth}
% %   \centering
% %   \includegraphics[scale=1,width=\textwidth]{bibtex/figures/encryption and app.png}
% %   \caption{\label{Fig:encryption and app}}
% %   \end{subfigure}
% %   \hspace{1mm}
%   \begin{subfigure}[b]{0.4\textwidth}
%   \centering
%   \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/connectivity and app.png}
%   \caption{\label{Fig:connectivity and app}}
%   \end{subfigure}
   
%   \begin{subfigure}[b]{0.4\textwidth}
%   \centering
%   \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/switching and app.png}
%   \caption{\label{Fig:switching and app}}
%   \end{subfigure}
%   \hspace{23mm}
%   \begin{subfigure}[b]{0.4\textwidth}
%   \centering
%   \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/reconfigurable logic and app.png}
%   \caption{\label{Fig:reconfigurable logic and app}}
%   \end{subfigure}
   
%   \caption{(a) Configurable buffer-inverter and Encrypted IC (b) Configurable routing and its application (c) Path switching and its application (d) Reconfigurable logic gates and its application\textcolor{red}{need revisit }}

% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[b]{0.4\textwidth}
%     \centering
%     \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/dynamic programming_1.png}
%   \caption{\label{Fig:dynamic programming_1}}
%     \end{subfigure}
%     \hspace{5mm}
%     \begin{subfigure}[b]{0.4\textwidth}
%     \centering
%     \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/peripheral programming_1.png}
%   \caption{\label{Fig:peripheral programming_1}}
%     \end{subfigure}
    
%     \caption{(a) Dynamic programming of encryption logic gates (b) Peripheral programming of encryption logic gates utilizing scan logic}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}[b]{0.4\textwidth}
%     \centering
%      \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/dynamic programming_2.png}
%      \caption{\label{Fig:dynamic programming_2}}
%     \end{subfigure}
%      \hspace{5mm}
%      \begin{subfigure}[b]{0.4\textwidth}
%      \centering
%      \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/peripheral programming_2.png}
%      \caption{\label{Fig:peripheral programming_2}}
%      \end{subfigure}
    
%     \caption{(a) Dynamic programming of encryption logic gates (b) Peripheral programming of encryption logic gates utilizing scan logic}
% \end{figure}



\begin{comment}
\begin{figure}
    \centering
    \includegraphics[scale=1,width=0.6\textwidth]{bibtex/figures/figure_programing.pdf}
    \caption{Caption}
    \label{fig:programming}
\end{figure}
\end{comment}

IP piracy and counterfeiting are the most serious security concerns to modern IC industry. A number of protection methods have been proposed \cite{HOST'13,SSP'17, HOST'08, DAC'09} in order to prevent circuits from attacking such as hardware Trojan and fault injection. Among them, camouflaging is a promising solution \cite{patent'01, patent'02, patent'03} which utilizes layout-level obfuscation for different gates with functionality and makes reverse engineering much difficult. 

Various gate-level camouflaging techniques have been developed with conventional CMOS devices \cite{Mai'16, ISSCC'18, ETS'16, HOST'18, ISLPED'18}. However, traditional CMOS-based camouflaging implementations incur the overhead and cost of high circuit complexity, area, power, and delay. With the development of emerging technology, more and more research has been concentrated on emerging devices in hardware security domain because of their unique properties and outstanding features such as spin-transfer-torque devices \cite{VLSI'14}, tunnel-FETs \cite{ESTCS'14} and ferroelectric devices incorporating with traditional devices \cite{ESTCS'15}.
\textcolor{blue}{ need more details here }

Rajendran et. al \cite{CCS'13} proposed a gate camouflaging technique by inserting dummy via/contacts in the layout and creating look-alike layouts for  NAND, NOR, and XNOR cells.  With layout look-alike camouflaged gates, the attackers may interpret the function incorrectly and end up with a faulty netlist. However, with the advance of modern computer visioning technology, such methods are less effective and can not resist direct probing of circuits \cite{Mai'16}. One approach to avoid this type of issue is to use internal parameters of devices for such as product invariability or different states of the devices to utilize identical physical layouts for implementing different functions.

Burak Erbagci et.al \cite{Mai'16} proposed a  gate camouflaging technique using threshold voltage defined (TVD) logic topology. The key idea of this approach relies on the usage of different threshold voltage transistors but with identical physical layouts. This work proposed a  generic 2-input TVD logic gate capable of realizing multiple logic functions (NAND, NOR, and XNOR) as shown in Fig. \ref{Fig:Prevwork}. They achieved this by setting pull down transistors with  different threshold implants( i.e. low-V$_T$ (LVT), and high-V$_T$ (LVT)). However, this circuit does not provide flexible reconfigurability as the threshold voltage of conventional CMOS transistors is not run-time programmable. 
 
 
 Sourav Dutta et. al. \cite{S_Datta_reconfig} further enhanced the TVD device design (Fig.~\ref{Fig:Prevwork}) by utilizing the threshold voltage programming property of the emerging device Ferroelectric FETs(FeFET). They replace the pull-down logic[Fig.~\ref{Fig:Prevwork}] with FeFETs. By utilizing the feature of voltage-dependent polarization switching of FeFET, Pull down transistors can be reprogrammed into LVT and HVT states. This makes the TVD logic gate-level camouflaging and run-time reconfigurable simultaneously. However, these features come at the expense of complex design with differential logic, high area, power, timing expense.  In our work, we propose a simple  area efficient logic which can act as key logic. We  utilize only two FeFETs to induce runtime reconfigurability of the logic. 
    In the next section, we describe details of the FeFET technology. 

\begin{comment}
To overcome the overhead of area, power and delay from  \cite{Mai'16}, Sourav Dutta et. al.~\cite{S_Datta_reconfig} proposed a novel FeFET-based TVD logic allowing gate-level camouflaging and run-time reconfigurability simultaneously. Moreover, they also implement an FeFET-based TVD logic topology which enables to implement any Boolean logic function not just NAND, NOR and XNOR~\cite{ISCAS'18, IEDM'171}. By utilizing the feature of voltage-dependent polarization switching of FeFET, FeFETs in camouflaged circuit can be reprogrammed as LVT and HVT states. Thus, their camouflaged circuit can achieve lower overhead because of run-time reconfigurability. Fig. x shows the schematic diagram of experimental set up and the measured waveforms are in Fig. x. ... However, this design still has some overhead such as area. Thus, we propose a novel ...
\end{comment}

\begin{comment}
\begin{figure}[]
\centering
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[scale=0.5,width=\columnwidth]{bibtex/figures/FeFET.png}
\caption{\label{Fig:FeFET}}
\end{subfigure}
\hspace{10mm}
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[scale=0.5,width=\columnwidth]{bibtex/figures/Vt.png}
\caption{\label{Fig:VT}}
\end{subfigure}
\hspace{10mm}
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[scale=0.8, width=\columnwidth]{bibtex/figures/reconf_circuit.png}
\caption{\label{Fig:reconfig}}
\end{subfigure}
\hspace{10mm}
\begin{subfigure}{0.3\columnwidth}
\centering
\includegraphics[scale=0.3, width=\columnwidth]{bibtex/figures/replace_prevwork.png}
\caption{\label{Fig:Prevwork}}
\end{subfigure}


\caption{(a) Structure of FeFET (b) Reconfigurable characteristics of FeFETs by applying programming voltages \textcolor{red}{Prof Kai s comment, For the Id-Vg curve, You do not need to show both the reset and set one as they are the same.will need to double check, exactly what he meant} (c) Our proposed reconfigurable encoding circuit with FeFET-based pass transistors (d) FeFET based generic 2 input TVD camouflage circuit. This circuit can can implement NOR NAND and XOR function \cite{Mai'16}.}
\end{figure}
\end{comment}

\begin{comment}
 So far, Various gate-level camouflaging techniques have been developed with conventional CMOS devices \cite{Mai'16, ISSCC'18, ETS'16, HOST'18, ISLPED'18}. However, traditional CMOS-based camouflaging implementations incur the overhead and cost of high circuit complexity, area, power and delay. With the development of emerging technology, more and more research has been concentrated on emerging devices in hardware security domain because of their unique properties and outstanding features such as spin-transfer-torque devices \cite{VLSI'14}, tunnel-FETs \cite{ESTCS'14} and ferroelectric devices incorporating with traditional devices \cite{ESTCS'15}.
Those methods will invariably cause increases in area and power consumption.

Traditional circuit encryption is to implement look-alike layout or insert dummy connection that interference with computer vision software.%Circuit camouflage integration for hardware IP protection
Those methods will cause increases in area and power consumption. 
With the advance of modern computer visioning technology, those methods are less effective and can not resist direct probing of circuits. If attackers directly measure the inputs and outputs of circuits, functions of the circuits can be easily determined.

One approach to avoid this type of issue is to use internal parameters of devices for such as product invariability or different state of the devices to utilize identical physical layout for implementing different functions.%A novel threshold voltage defined switch for circuit camouflaging
Another approach is by inserting dummy nets.%circuiting analysis of integrated circuit camouflaging
By inserting traces on the metal layer and connecting them with the hollow vias, attackers cannot easily use computer imaging to determine connection topologys. This method can realize 3 functions with ~5x power and area overheads%A novel threshold voltage defined witch for circuit camafluging.
and cannot resist direct measurement for circuits. Attackers can directly send excitation signals and measure outputs in order to reverse engineering the netlist. 

\textcolor{red}{February security previs vt paper and other security paper
normal state
advantage of our technology use less transistor}
\end{comment}

\begin{comment}
\begin{figure}[ht]
  \centering
  \begin{subfigure}[b]{0.5\textwidth}
  \centering
  \includegraphics[scale=0.4,width=\textwidth]{bibtex/figures/encryption and app.png}
   \caption{\label{Fig:encryption and app}}
   \end{subfigure}
   \hspace{10mm}
   \begin{subfigure}[b]{0.4\textwidth}
   \centering
   \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/connectivity and app.png}
   \caption{\label{Fig:connectivity and app}}
   \end{subfigure}
   
   \begin{subfigure}[b]{0.4\textwidth}
  \centering
  \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/switching and app.png}
   \caption{\label{Fig:switching and app}}
   \end{subfigure}
   \hspace{23mm}
   \begin{subfigure}[b]{0.4\textwidth}
   \centering
   \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/reconfigurable logic and app.png}
   \caption{\label{Fig:reconfigurable logic and app}}
   \end{subfigure}
   
   \caption{(a) Configurable buffer-inverter and Encrypted IC (b) Configurable routing and its application (c) Path switching and its application (d) Reconfigurable logic gates and its application\textcolor{red}{need revisit }}

\end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.8\textwidth}
    \centering
    \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/dynamic programming_1.png}
    \caption{\label{Fig:dynamic programming_1}}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.8\textwidth}
    \centering
    \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/peripheral programming_1.png}
    \caption{\label{Fig:peripheral programming_1}}
    \end{subfigure}
    
    \caption{(a) Dynamic programming of encryption logic gates (b) Peripheral programming of encryption logic gates utilizing scan logic}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.8\textwidth}
    \centering
    \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/dynamic programming_2.png}
    \caption{\label{Fig:dynamic programming_2}}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.8\textwidth}
    \centering
    \includegraphics[scale=0.5,width=\textwidth]{bibtex/figures/peripheral programming_2.png}
    \caption{\label{Fig:peripheral programming_2}}
    \end{subfigure}
    
    \caption{(a) Dynamic programming of encryption logic gates (b) Peripheral programming of encryption logic gates utilizing scan logic}
\end{figure}
\end{comment}

==> bibtex/sections/previus_work.tex <==
\section*{Related works}


IP piracy and counterfeiting are the most serious security concerns to modern IC industry. A number of protection methods have been proposed\textcolor{verify}{\cite{HOST'13,SSP'17, HOST'08, DAC'09}} in order to prevent hardware attacks. Among them, camouflaging is a promising solution \cite{patent'01, patent'02, patent'03} which utilizes layout-level obfuscation for different gates with functionality and makes reverse engineering much difficult. 

Various gate-level camouflaging techniques have been developed with conventional CMOS devices\cite{Mai'16, ISSCC'18, ETS'16, HOST'18, ISLPED'18}. However, traditional CMOS-based camouflaging implementations incur the overhead and cost of high circuit complexity, area, power, and delay. With the development of emerging technology, more and more research has been concentrated on emerging devices in hardware security domain due to their unique properties such as CMOS compatibility, scalability, energy efficiency etc. Devices  such as  spin-transfer-torque devices\cite{VLSI'14}, tunnel-FETs \cite{ESTCS'14},ferroelectric devices \cite{ESTCS'15},\textcolor{red}{previous nature security device}, etc., have been studied in this aspect \textcolor{red}{double check citation}.


Jeyavijayan Rajendran et al.\cite{CCS'13} proposed a gate camouflaging technique by inserting dummy via/contacts in the layout and creating look-alike layouts for  NAND, NOR, and XNOR cells (Fig.~\ref{fig:overview}(c)).  With layout look-alike camouflaged gates, the attackers may interpret the function incorrectly and end up with a faulty netlist. However, with the advance of modern computer visioning technology, such methods are less effective and can not resist direct probing of circuits\cite{Mai'16}. One approach to avoid this type of issue is to use internal parameters of devices for such as product invariability or different states of the devices to utilize identical physical layouts for implementing different functions.

Burak Erbagci et al. \cite{Mai'16} proposed a  gate camouflaging technique using threshold voltage defined (TVD) logic topology. The key idea of this approach relies on the usage of different threshold voltage transistors but with identical physical layouts. This work proposed a  generic 2-input TVD logic gate capable of realizing multiple logic functions (NAND, NOR, and XNOR). They achieved this by setting pull down transistors with  different threshold implants( i.e. low-V$_T$ (LVT), and high-V$_T$ (HVT)). However, this circuit does not provide flexible reconfigurability as the threshold voltage of conventional CMOS transistors is not run-time programmable. 
 
 Peng Wu et al.\cite{2D-polarity} proposed that two-dimensional black phosphorus field-effect transistors that have reconfigurable polarities are suitable for hardware security applications (Fig.~\ref{fig:overview}(c)). The transistors can be dynamically switched between p-FET and n-FET operation through electrostatic gating. And it achieves minimum area overhead. However, this kind of design is incompatible with Si-CMOS technology.
 
 
 Sourav Dutta et al.\cite{S_Datta_reconfig} further enhanced the TVD device design (Fig.~\ref{fig:overview}(c)) by utilizing the threshold voltage programming property of the emerging device Ferroelectric FETs (FeFETs). They replace the pull-down logic with FeFETs. By utilizing the feature of voltage-dependent polarization switching of FeFET, Pull down transistors can be reprogrammed into LVT and HVT states. This makes the TVD logic gate-level camouflaging and run-time reconfigurable simultaneously. However, these features come at the expense of complex design with differential logic, high area, power, timing expense.  In our work, we propose a simple  area efficient logic which can act as key logic. We  utilize only two FeFETs to induce runtime reconfigurability of the logic. Also the aforementioned works have not explored the implementation of programming logic. In this we work, we present a scan based provision for programming the keybits. 

 
 In the next section, we describe details of the proposed interconnect based encryption block. 



==> bibtex/sections/reconfiganalysis.tex <==

%\section*{ Reconfigurable Logic}

%it is a good idea \cite{Loh1}

\begin{comment}
\begin{figure}
\centering
  
  \hspace{10mm}
  \begin{minipage}{\textwidth}
  \centering
   \captionof{table}{Truth table of 3-State camouflaging circuit \textcolor{red}{add CNTL1 and CNTL2 also}}
  \begin{tabular}{|c|c|c|c|c|}
    \hline
     INPUT1   &  INPUT2 & XOR (C1=BUF, C2=BUF) & OR(C1=INV, C2=INV) & XNOR(C1=BUF, C2=INV) \\
    \hline
    0 & 0 & 0 & 0 & 1 \\
    \hline
    0 & 1 & 1 & 1 & 0 \\
    \hline
    1 & 0 & 1 & 1 & 0 \\
    \hline
    1 & 1 & 0 & 1 & 1 \\
    \hline
    \end{tabular}
   
    \label{tab:truth table of XOR_camouflage}
  \end{minipage}
  
\end{figure}
\end{comment}

%\subsection{Reconfigurable circuits}
%Dummy interconnect are metal layers that are two metals that appears to be connected to reverse engineer. To implement this, a pass tansistor is placed in between two metal traces. The true interconnect will be the coneection that FeFET programmed to low Vt state so the metal trace is continuous. Then for a dummy net, the pass FeFET is programmed into high Vt state so the circuit will act as a fuse to disconnect the connection. Fig x.
Reconfigurable \label{Reconfigurable} logic is a known camouflaging method  to obfuscate the IP. Here the attacker will not be able to discern the logic and extract the correct netlist by observing the layout. Standard cell is the building block in ICs for logic operations. The more functions it has with the same layout, the harder to be attacked. The active interconnect based encryption gate can be used in conjunction with standard cells to make a very easy implementable reconfigurable logic. 
%The easiest and simplest two-state implantation is to put the encryption circuit on the output of standard cell to camouflage the original circuit. 
An example is shown with NAND gate in \textcolor{red}{Fig.~\ref{fig:figure4_propagation}(e)}.   Instantiating encryption logic in the inverter mode to the output of NAND gate make the combination "AND" gate. Adding  encryption circuit to the inputs of NAND gates makes it further programmable. 
This makes the combination reconfigurable to NOR/OR. The internal programmed state of the instantiated interconnect based logic  and potential logic gates centered around NAND gate are shown in \textcolor{blue}{ supplementary material Table.~\ref{fig:truth table of NAND}}.  

%By adding a security logic on the output and input of the circuit, the new camouflaged circuit is able to program into NAND gate and AND gate with only 2x area overhead compared to a 4T NAND gate. We can make it further programmable by adding proposed encryption circuit to the inputs of NAND gates as Fig.~\ref{fig:figure4_propagation}d shown. By inverting both input and output of NAND gate, we can effectively make this circuit behave as an OR or NOR gate and get a three state camoflaged standard cell.

\begin{comment}
The easiest and simplest two-state implantation is to put the encryption circuit on the output of standard cell to camouflage the original circuit and its complement logic. We can modify NAND as such gate has the number of transistors (16T). By adding a security logic on the output of the circuit, the new camouflaged circuit is able to program into XOR gate and XNOR gate with only 1.25x overhead compared to a 16T XOR gate. To maximize the security of our circuit, we can place additional encryption gates in the inputs of XOR as well.  For example adding one encryption in the input of XOR and one at the output of XOR , the combination can act as OR gate (\textcolor{red}{doesnt seem to be right}. The truth table is given in Table.~\ref{tab:truth table of NAND_camouflage}. The area overhead of such circuit would be 1.5x.


the proposed security logic on one of the input and output of the XNOR gate as Fig.~\ref{fig:figure4_propagation}(d) shown. By inverting one input of XNOR gate, we can effectively make this circuit behave as an OR gate. If we add two proposed circuits on the output and an input of XOR gate, we will get a circuit that can preform XOR, XNOR or OR operations depending on programming states. 

The proof follows: By definition, \[A \oplus B = \overline{A}*B + A\overline{B}\] then, for our circuit, \[\overline{\overline{A} \oplus B} = \overline{\overline{\overline{A}}*B + \overline{A}\overline{B}}\]  \[\overline{\overline{A} \oplus B} = \overline{A*B + \overline{A}\overline{B}}\] then we apply DeMorgan's law and simplify, \[\overline{\overline{A} \oplus B} = \overline{\overline{A}+\overline{B}+\overline{A}+\overline{B}}\] \[\overline{\overline{A} \oplus B} = A + B \]Hence,   
\end{comment}

%dIn order to further To to implement a A OR B we can perform A XNOR NOT B overhead 1.66x  %we need to prooof the logic, thould have XNOR XOR and AND state, I'm workoing on the proof now) 

%% Comment Sumitha : I feel if we have enoguh content then we can put the dummy configurable gate as another journal  paper. In that way we are doubleing number of papers
% sure, dont delete now, just comment the lines.so that if we require, it is there.

%Ok, I will keep it on there for now as comment. Also lines below may need to be deleted since we are not using AND gate as base also AND encryption does have large area penalty. 



%Need to revisit this

%There are three placement configurations for proposed circuit: Stand Cell Encryption, Interconnect Encryption and Output Encryption.   
%o encrypt a standard cell, we can connect proposed circuit the on all the terminals of a standard AND gate as Figx shown. This circuit can realises AND NAND NOR and OR gate. For AND configuration, all three encryption circuits are set into buffer mode and the base and gate will not be altered. For a NAND gate, output of base AND gate will be configured as a inverts. For NOR gate configuration, we can set to invert both inputs of the AND gate due to Demorgan's law of \[\bar{A} * \bar{B} = \overline{A+B}\].The same can be obtained for OR gate by setting bothe input and the out put for the base AND gate as an inverter. 

%To Encrypt interconnects,  Designer can insert dummy connection in metal layer, those connection can connect to a Ferroelectirc pass transistor along with the real connection. The pass transistors for dummy connection will be programmed into high Vt state and act as a fuse.
\begin {comment}
\textcolor{blue}{the below paragrpah may move to supplemental section}

All the above techniques often increase the reliability against the attacker. Since the operation of the logic cell is hidden by the attacker, reverse engineering can only be done by measuring output of the circuit. However with the number of inputs and depending on the position and logic nature of the the decoding, the encryption becomes a hard problem. 
Table.~\ref{tab:truth table of NAND_camouflage} is the truth table for 4 \textcolor{red}{state} camouflage logic. In order to determine the state of the circuit, the attacker needs to brute force all 4 possible inputs and uses the Karnaugh-map method to determine encrypted logic. If attacker incorrectly determined state of the circuit, for example, attacker determined the circuit is NAND gate instead of correct OR gate, the circuit would generate incorrect output for 3 out of 4 input patterns. 
Jeyavijayan Rajendran et al.\cite{CCS'13} shows that placement of camouflaging gates at specific locations ensure the output of the extracted netlist, resistant to  reverse engineering.
\end{comment}
%Although it sounds simple, if the encryption bit is not placed correctly, undetermined bit may not able propagate due to the logic masking effect. As for a simplified two input logic, if only one input is encrypted, it is possible to reverse engineering the output form another input. 
%Logic For example the circuit using in Fig. \ref{Fig:position-3}, if input I3 is 0, the in-determined bit can propagate to the output. If input I3 is changed to 1, the OR gate will block the indeterminate bit and get the correct output. So this circuit only has encrypted bits for 8 of 16 possible inputs.

%\textcolor{red}{
%explain in terms of reverse engineering, how our circuit is reliable,
 %The first talk about how to reverse engineering the logic by directly measuring the output from input stimulation. The time complexity would be exponential. }

==> bibtex/sections/security.tex <==
\section*{security}


Traditional  circuit encryption is to implement look-alike layout or insert dummy connection that interference with computer vision software.%Circuit camouflage integration for hardware IP protection
Those method will cause increase in area and power consumption. With the advance of modern computer visioning technology, those method are less effective and those method can not resist direct probing of the circuit. If the attacker directly measures the input and the output of the circuit, function of the circuit can be easily determined. One approach is to use the internist parameter of the device for such as product invariability or different state of the devices to utilize identical layout for implementing different fictions.%A novel threshold voltage defined switch for circuit camouflaging
Another approach is by inserting dummy net.%circuiting analysis of integrated circuit camouflaging
By inserting traces on the metal layer and connect them with the hollow vias, attacker can not easily use computer imaging to determined connection topology. This method can realize 3 functions at ~5x power and area overhead%A novel threshold voltage defined witch for circuit camafluging.
and can not resist direct measurement for the circuit. Attacker can directly send excitation signal and measure the output to reverse engineer the netlist. 



February security previs vt paper and other security paper
normal state
advantage of our technology use less transistor

